Anticipating Technical Expertise and Capability Evolution in Research Communities using Dynamic Graph Transformers

The ability to anticipate technical expertise and capability evolution trends globally is essential for national and global security, especially in safety-critical domains like nuclear nonproliferation (NN) and rapidly emerging fields like artificial intelligence (AI). In this work, we extend traditional statistical relational learning approaches (e.g., link prediction in collaboration networks) and formulate a problem of anticipating technical expertise and capability evolution using dynamic heterogeneous graph representations. We develop novel capabilities to forecast collaboration patterns, authorship behavior, and technical capability evolution at different granularities (e.g., scientist and institution levels) in two distinct research fields. We implement a dynamic graph transformer (DGT) neural architecture, which pushes the state-of-the-art graph neural network models by (a) forecasting heterogeneous (rather than homogeneous) nodes and edges, and (b) relying on both discrete -- and continuous -- time inputs. We demonstrate that our DGT models predict collaboration, partnership, and expertise patterns with 0.26, 0.73, and 0.53 mean reciprocal rank values for AI and 0.48, 0.93, and 0.22 for NN domains. DGT model performance exceeds the best-performing static graph baseline models by 30-80% across AI and NN domains. Our findings demonstrate that DGT models boost inductive task performance, when previously unseen nodes appear in the test data, for the domains with emerging collaboration patterns (e.g., AI). Specifically, models accurately predict which established scientists will collaborate with early career scientists and vice-versa in the AI domain.

==> sections/results_presentation.tex <==

\ignore{
\begin{table*}[htbp]
\caption{Forecasting performance in transductive and inductive settings. We label source-to-target relationships with seen and unseen nodes during training. The seen-to-seen relationships are grouped into first-time and repeated interactions. \textbf{First}, \textbf{Second}, \textbf{Third} best performing methods are in bold. $\dagger$ Does not support inductive
% \shnote{Ana, update the table.}
}

\begin{tabular}{|c|c|rr|r|}
\hline
\multirow{3}{*}{Domain} & \multirow{3}{*}{Model} & \multicolumn{2}{c|}{Transductive}                                                             & \multicolumn{1}{c||}{Inductive}                      
                     %& \multicolumn{2}{c|}{True Inductive}   
                     \\ \cline{3-5} 
                       & & \multicolumn{1}{c|}{Seen-to-Seen (First-Time)} & \multicolumn{1}{c|}{Seen-to-Seen (Repeated)} & \multicolumn{1}{c||}{Unseen-to-Seen} \\ \cline{3-5} %& \multicolumn{1}{c|}{Seen-to-Unseen} & \multicolumn{1}{c|}{Unseen-to-Unseen} \\ \cline{3-7} 
                       && \multicolumn{1}{c|}{MRR} &  \multicolumn{1}{c|}{MRR} &  \multicolumn{1}{c||}{MRR} \\ \hline %& \multicolumn{1}{c|}{Avg. Precision} & \multicolumn{1}{c|}{Avg. Precision} \\ \hline
                       \hline
\multirow{10}{*}{ACL}    & TransE                 & \multicolumn{1}{r|}{0.084284}                  & 0.130113                                     & \multicolumn{1}{r|}{$\dagger$}    \\ \cline{2-5}           %& \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
 & RotatE                 & \multicolumn{1}{r|}{0.095328}                  & 0.132924                                     & \multicolumn{1}{r|}{$\dagger$}          \\ \cline{2-5}    % & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
 & ConvE                  & \multicolumn{1}{r|}{0.005433}                  & 0.005568                                     & \multicolumn{1}{r|}{$\dagger$}              \\ \cline{2-5} % & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
 & ComplEx                & \multicolumn{1}{r|}{0.058125}                  & 0.067563                                     & \multicolumn{1}{r|}{$\dagger$}               \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
 & RGCN                   & \multicolumn{1}{r|}{0.099215}                  & 0.165076                                     & \multicolumn{1}{r|}{$\dagger$}              \\ \cline{2-5} % & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & NodePiece              & \multicolumn{1}{r|}{0.005441}                  & 0.005664                                     & \multicolumn{1}{r|}{$\dagger$}               \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
 & RENet                  & \multicolumn{1}{r|}{\textbf{0.325359}}                  & \textbf{0.527458}                                     & \multicolumn{1}{r|}{0.030452}      \\ \cline{2-5} % & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
 & TGN                    & \multicolumn{1}{r|}{0.217575}                  & 0.247502                                     & \multicolumn{1}{r|}{\textbf{0.215161}}      \\ \hline \hline % & \multicolumn{1}{r|}{\shnote{*}}               &                                       \multicolumn{1}{r|}{\shnote{*}}  \\ \cline{2-7}
%  & DGT-D                  & \multicolumn{1}{r|}{\textbf{0.313757}}                 & \textbf{0.521902}                                     & \multicolumn{1}{r|}{0.030976}      \\ \cline{2-5} % & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & DGT-C                  & \multicolumn{1}{r|}{\textbf{0.494414}}                  & \textbf{0.616278}                                     & \multicolumn{1}{r|}{\textbf{0.487087}}      \\ \hline \hline%\\ \cline{2-5} % & \multicolumn{1}{r|}{\shnote{*}}               &                                       \multicolumn{1}{r|}{\shnote{*}}  \\ \hline
 \hline
 %%%%
 %%%%
 %%%%
%   \multirow{10}{*}{ICLR}    & TransE                 & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & RotatE                 & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & ConvE                  & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & ComplEx                & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & RGCN                   & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & NodePiece              & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & RENet                  & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & TGN                    & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & DGT-D                  & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & DGT-C                  & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \hline \hline
 %%%%
 %%%%
 %%%%
%   \multirow{10}{*}{ICML}    & TransE                 & \multicolumn{1}{r|}{} & & \multicolumn{1}{r|}{$\dagger$} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
% & RotatE                  & \multicolumn{1}{r|}{} & & \multicolumn{1}{r|}{$\dagger$} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & ConvE                  & \multicolumn{1}{r|}{} & & \multicolumn{1}{r|}{$\dagger$} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & ComplEx                & \multicolumn{1}{r|}{} & & \multicolumn{1}{r|}{$\dagger$} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & RGCN                   & \multicolumn{1}{r|}{} & & \multicolumn{1}{r|}{$\dagger$} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & NodePiece              & \multicolumn{1}{r|}{} & & \multicolumn{1}{r|}{$\dagger$} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & RENet                  & \multicolumn{1}{r|}{} & & \multicolumn{1}{r|}{} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & TGN                    & \multicolumn{1}{r|}{} & & \multicolumn{1}{r|}{} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & DGT-D                 & \multicolumn{1}{r|}{} & & \multicolumn{1}{r|}{} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & DGT-C                 & \multicolumn{1}{r|}{} & & \multicolumn{1}{r|}{} \\ \hline \hline%\\ \cline{2-5} % \\ \hline%& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \hline \hline
%  \hline
 %%%%
 %%%%
 %%%%
 \multirow{10}{*}{WoS}    & TransE                 & \multicolumn{1}{r|}{0.059885}                  & 0.113255                                    & \multicolumn{1}{r|}{$\dagger$}               \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
 & RotatE                 & \multicolumn{1}{r|}{0.063733}                  & 0.123397                                     & \multicolumn{1}{r|}{$\dagger$}              \\ \cline{2-5} % & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
 & ConvE                  & \multicolumn{1}{r|}{0.005664}                  & 0.005633                                     & \multicolumn{1}{r|}{$\dagger$}               \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
 & ComplEx                & \multicolumn{1}{r|}{0.048307}                  & 0.094574                                     & \multicolumn{1}{r|}{$\dagger$}               \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
 & RGCN                   & \multicolumn{1}{r|}{0.078822}                  & 0.161568                                     & \multicolumn{1}{r|}{$\dagger$}               \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & NodePiece              & \multicolumn{1}{r|}{0.005780}                  & 0.006248                                    & \multicolumn{1}{r|}{$\dagger$}               \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
 & RENet                  & \multicolumn{1}{r|}{\textbf{0.310669}}                  & \textbf{0.671367}                                     & \multicolumn{1}{r|}{0.021093}       \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
 & TGN                    & \multicolumn{1}{r|}{0.150731}                  & 0.198640                                    & \multicolumn{1}{r|}{\textbf{0.138444}}       \\ \cline{2-5} %& \multicolumn{1}{r|}{\shnote{*}}               &                                       \multicolumn{1}{r|}{\shnote{*}}  \\ \cline{2-7}
%  & DGT-D                  & \multicolumn{1}{r|}{\textbf{0.294672}}                  & \textbf{0.648270}                                    & \multicolumn{1}{r|}{0.020726}       \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & DGT-C                  & \multicolumn{1}{r|}{\textbf{0.200879}}                  & \textbf{0.246949}                                    & \multicolumn{1}{r|}{\textbf{0.170331}}       \\ \hline \hline %\ \cline{2-5} %& \multicolumn{1}{r|}{\shnote{*}}               &                                       \multicolumn{1}{r|}{\shnote{*}}  \\ \hline \hline
 \hline
 %%%%
 %%%%
 %%%%
%  \multirow{10}{*}{Scopus}    & TransE                 & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & RotatE                 & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & ConvE                  & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & ComplEx                & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & RGCN                   & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & NodePiece              & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & RENet                  & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & TGN                    & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & DGT-D                  & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & DGT-C                  & \multicolumn{1}{r|}{}                  &                                     & \multicolumn{1}{r|}{$\dagger$}               & \multicolumn{1}{r|}{$\dagger$}               &                                       \multicolumn{1}{r|}{$\dagger$}  \\ \hline \hline
%  \multirow{10}{*}{Scopus}    & TransE                 & \multicolumn{1}{r|}{0.086030} & 0.092914 & \multicolumn{1}{r|}{$\dagger$} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
% & RotatE                  & \multicolumn{1}{r|}{0.086876} & 0.094809 & \multicolumn{1}{r|}{$\dagger$} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & ConvE                  & \multicolumn{1}{r|}{0.012684} & 0.013350 & \multicolumn{1}{r|}{$\dagger$} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & ComplEx                & \multicolumn{1}{r|}{0.079884} & 0.085138 & \multicolumn{1}{r|}{$\dagger$} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & RGCN                   & \multicolumn{1}{r|}{0.148987} & 0.197054 & \multicolumn{1}{r|}{$\dagger$} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & NodePiece              & \multicolumn{1}{r|}{0.006314} & 0.006658 & \multicolumn{1}{r|}{$\dagger$} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & RENet                  & \multicolumn{1}{r|}{0.617189} & 0.824981 & \multicolumn{1}{r|}{0.025419} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & TGN                    & \multicolumn{1}{r|}{0.189512} & 0.228042 & \multicolumn{1}{r|}{0.107457} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & DGT-D                 & \multicolumn{1}{r|}{0.600000} & 0.816609 & \multicolumn{1}{r|}{0.025032} \\ \cline{2-5} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  \\ \cline{2-7}
%  & DGT-C                 & \multicolumn{1}{r|}{0.162922} & 0.185909 & \multicolumn{1}{r|}{0.215255} %& \multicolumn{1}{r|}{$\dagger$} & \multicolumn{1}{r|}{$\dagger$}  
%  \\ \hline \hline
\end{tabular}
\end{table*}
}









